A Uniform Language to Explain Decision Trees

The formal XAI community has studied a plethora of interpretability queries aiming to understand the classifications made by decision trees. However, a more uniform understanding of what questions we can hope to answer about these models, traditionally deemed to be easily interpretable, has remained elusive. In an initial attempt to understand uniform languages for interpretability, Arenas et al. (2021) proposed FOIL, a logic for explaining black-box ML models, and showed that it can express a variety of interpretability queries. However, we show that FOIL is limited in two important senses: (i) it is not expressive enough to capture some crucial queries, and (ii) its model agnostic nature results in a high computational complexity for decision trees. In this paper, we carefully craft two fragments of first-order logic that allow for efficiently interpreting decision trees: Q-DT-FOIL and its optimization variant OPT-DT-FOIL. We show that our proposed logics can express not only a variety of interpretability queries considered by previous literature, but also elegantly allows users to specify different objectives the sought explanations should optimize for. Using finite model-theoretic techniques, we show that the different ingredients of Q-DT-FOIL are necessary for its expressiveness, and yet that queries in Q-DT-FOIL can be evaluated with a polynomial number of queries to a SAT solver, as well as their optimization versions in OPT-DT-FOIL. Besides our theoretical results, we provide a SAT-based implementation of the evaluation for OPT-DT-FOIL that is performant on industry-size decision trees.

==> new-sections/proof-poly-order.tex <==

\section{Proof of Theorem \ref{}}

Let $\rho[v_1, \ldots, v_\ell](x,y)$ be a formula that represents a
strict partial order. Then a sequence $(\es_1, \ldots, \es_k)$ of
partial instantes is a path of dimension $n$ in $\rho[v_1, \ldots,
  v_\ell](x,y)$ if $\es_i$ is a partial instance of dimension $n$ for
each $i \in \{1, \ldots, k\}$, and there exist a decision tree $\T$ of
dimension $n$ and instances $\es'_1$, $\ldots$, $\es'_\ell$ of
dimension $n$ such that $\T \models \rho[\es'_1, \ldots,
  \es'_\ell](\es_i,\es_{i+1})$ for every $i \in \{1, \ldots,
k-1\}$. 

\begin{lemma}\label{lem-fixed-rho}
Fix a formula $\rho[v_1, \ldots, v_\ell](x,y)$ that represents a
strict partial order. Then there exists a fixed polynomioal $p$ such
that for every path $(\es_1, \ldots, \es_k)$ of dimension $n$ in
$\rho[v_1, \ldots, v_\ell](x,y)$, it holds $k \leq p(n)$.
\end{lemma}

\begin{proof}
First, we consider a formula that represents a strict partial order of
the form $\rho(x,y)$, and then we extend the proof to the case of a
formula $\rho[v_1, \ldots, v_\ell](x,y)$ with parameters $v_1$,
$\ldots$, $v_\ell$.

Fix a dimension $n$ and a decision tree $\T$ of dimension $n$, and assume that
$\mathfrak{B}_\T$ is a structure over the vocabulary $\{\subseteq,
\preceq\}$ generated from $\T$ by removing the interpretation of the
predicate $\pos$. Then given a partial instance of dimension $n$,
define $\#_0(\es)$ as the number of occurances of the symbol $0$ in
$\es$, and likewise for $\#_1(\es)$ and $\#_\bot(\es)$. Moreover, for
every $(p,q,r) \in \mathbb{N}^3$ such that $p + q + r = n$, define
\begin{align*}
  L_{(p,q,r)} \ = \ \{ \es \mid \es \text{ is a partial instance of
    dimension } n \text{ such that } \#_0(\es) = p,\, \#_1(\es) = q
  \text{ and } \#_\bot(\es) = r \}.
\end{align*}
Notice that there are at most $(n+1)^3$ sets $L_{(p,q,r)}$. In what
follows, we shows that if $\es_1$ and $\es_2$ are two distinct partial
instances of dimension $n$ such that $\es_1 \in L_{(p,q,r)}$ and
$\es_2 \in L_{(p, q, r)}$, then $\T \not\models \rho(\es_1,
\es_2)$. From this we conclude that the statement of the lemma holds
for $p(n) = (n+1)^3$, since if $(\es_1, \ldots, \es_k)$ is a path of
dimension $n$ in $\rho(x,y)$, then each $\es_i$ must belong to a
different set $L_{(p,q,r)}$.

For the sake of contradiction, assume that $\es_1 \neq \es_2$, $\es_1
\in L_{(p, q, r)}$, $\es_2 \in L_{(p,q,r)}$, and $\T \models
\rho(\es_1, \es_2)$. Given that $\es_1 \in L_{(p, q, r)}$ and $\es_2
\in L_{(p,q,r,)}$, there exists a permutation $\pi : \{1, \ldots, n\}
\to \{1, \ldots, n\}$ such that $\pi(\es_1) = \es_2$. For every pair
$\es$, $\es'$ of partial instances of dimension $n$, it holds that:
\begin{align*}
  \es \subseteq \es' &\quad\quad\Leftrightarrow\quad\quad   \pi(\es) \subseteq \pi(\es')\\
  \es \preceq \es' &\quad\quad\Leftrightarrow\quad\quad   \pi(\es) \preceq \pi(\es').
\end{align*}
Hence, $\pi$ is an automorphism for the structure $\mathfrak{B}_\T$,
from which we conclude that $\mathfrak{B}_\T \models \rho(\pi(\es_1),
\pi(\es_2))$ given that $\rho$ is a formula defined over the
vocabulary $\{ \subseteq, \preceq\}$ and $\T \models \rho(\es_1 ,
\es_2)$. Thus, we have that $\T \models \rho(\pi(\es_1), \pi(\es_2))$
and, therefore, $\T \models \rho(\es_1, \pi^2(\es_1))$ since $\es_2 =
\pi(\es_1)$ and $\rho(x, y)$ represents a strict partial order. In the
same way, it is possible to conclude that $\T \models \rho(\es_1,
\pi^k(\es_1))$ for every $k \geq 1$. Given that the set of
permutations of $n$ elements with the composition operator forms a
group of order $n!$, we know that $\pi^{n!}$ is the identity
permuntation, so that $\pi^{n!}(\es_1) = \es_1$. Therefore, we
conclude that $\T \models \rho(\es_1, \es_1)$, which leads to a
contradiction since $\rho(x,y)$ represents a strict partial order.


Consider now a formula $\rho[v_1, \ldots, v_\ell](x,y)$ that
represents a strict partial order. As in the previous case without
parameters, fix a dimension $n$ and a decision tree $\T$ of dimension
$n$, and assume that $\mathfrak{B}_\T$ is a structure over the
vocabulary $\{\subseteq, \preceq\}$ generated from $\T$ by removing
the interpretation of the predicate $\pos$. Moreover, fix a sequence
$\es'_1$, $\ldots$, $\es'_\ell$ of instances of dimension $n$. Then,
for every $(a_1, \ldots, a_\ell) \in \{0,1,\bot\}^\ell$ and every
partial instance $\es$ of dimension $n$, define
\begin{align*}
  P_{(a_1, \ldots, a_\ell)} \ = \ \{i \in \{1, \ldots, n\} \mid \forall j \in \{1, \ldots, \ell\} \,:\, \es'_j[i] = a_i\}
\end{align*}
and
\begin{align*}
  \#_{(0, a_1, \ldots, a_\ell)}(\es) \ = \ |\{ i \in P_{(a_1, \ldots,
    a_\ell)} \mid \es[i]=0 \}|.
\end{align*}
That is, $\#_{(0, a_1, \ldots, a_\ell)}(\es)$ is the number of
occurances of the symbol $0$ in $\es$ among the positions $P_{(a_1,
  \ldots, a_\ell)}$. The functions $\#_{(1, a_1, \ldots,
  a_\ell)}(\es)$ and $\#_{(\bot, a_1, \ldots, a_\ell)}(\es)$ are
defined in the same way. Finally, consider an arbitrary enumeration
$t_1$, $\ldots$, $t_{3^\ell}$ of the tuples in
$\{0,1,\bot\}^\ell$, and for every $(p_1, q_1, r_1, \ldots,
p_{3^\ell}, q_{3^\ell}, r_{3^\ell}) \in \mathbb{N}^{3^{\ell + 1}}$
define
\begin{multline*}
  L_{(p_1, q_1, r_1, \ldots, p_{3^\ell}, q_{3^\ell},r_{3^\ell})} \ =
  \ \{ \es \mid \es \text{ is a partial instance of dimension } n
  \text{ such that }\\ \#_{(0,t_i)}(\es) = p_i, \#_{(1,t_i)}(\es) =
  q_i, \text{ and } \#_{(\bot,t_i)}(\es) = r_i \text{ for every } i
  \in \{1, \ldots, 3^{\ell} \} \}.
\end{multline*}
Notice that there are at most $(n+1)^{3^{\ell + 1}}$ sets $L_{(p_1,
  q_1, r_1, \ldots, p_{3^\ell}, q_{3^\ell},r_{3^\ell})}$. In what
follows, we shows that if $\es_1$ and $\es_2$ are two distinct partial
instances of dimension $n$ such that $\es_1 \in L_{(p_1, q_1, r_1,
  \ldots, p_{3^\ell}, q_{3^\ell},r_{3^\ell})}$ and $\es_2 \in L_{(p_1,
  q_1, r_1, \ldots, p_{3^\ell}, q_{3^\ell},r_{3^\ell})}$, then $\T
\not\models \rho[\es'_1, \ldots, \es'_\ell](\es_1, \es_2)$. From this
we conclude, as in the previous case without parameters, that the
statement of the lemma holds for $p(n) = (n+1)^{3^{\ell+1}}$, as
$\ell$ is a fixed number since the formula $\rho[v_1, \ldots,
  v_\ell](x,y)$ is assumed to be fixed.


For the sake of contradiction, assume that $\es_1 \neq \es_2$, $\es_1
\in L_{(p_1, q_1, r_1, \ldots, p_{3^\ell}, q_{3^\ell},r_{3^\ell})}$,
$\es_2 \in L_{(p_1, q_1, r_1, \ldots, p_{3^\ell},
  q_{3^\ell},r_{3^\ell})}$, and $\T \models \rho[\es'_1, \ldots,
  \es'_\ell](\es_1, \es_2)$. Given that $\es_1 \in L_{(p_1, q_1, r_1,
  \ldots, p_{3^\ell}, q_{3^\ell},r_{3^\ell})}$ and $\es_2 \in L_{(p_1,
  q_1, r_1, \ldots, p_{3^\ell}, q_{3^\ell},r_{3^\ell})}$, there exist
permutations $\pi_i : P_{t_i} \to P_{t_i}$ for $i \in \{1, \ldots,
3^{\ell}\}$ such that the permutation $\pi : \{1, \ldots, n\} \to \{1,
\ldots, n\}$ obtained by combining them satisfies that $\pi(\es_1) =
\es_2$. Notice that by definition of the permutations $\pi_i$ and the
sets $P_{t_i}$, we have that $\pi(\es'_j) = \es'_j$ for every $j \in
\{1, \ldots, \ell\}$.



As in the previous case without parameters, we have that $\pi$ is an
automorphism for the structure $\mathfrak{B}_\T$. Hence, we have that
$\mathfrak{B}_\T \models \rho[\pi(\es'_1), \ldots,
  \pi(\es'_\ell)](\pi(\es_1), \pi(\es_2))$ given that $\rho$ is a
formula defined over the vocabulary $\{ \subseteq, \preceq\}$ and $\T
\models \rho[\es'_1, \ldots, \es'_\ell](\es_1 , \es_2)$. Thus, we have
that $\T \models \rho[\pi(\es'_1), \ldots,
  \pi(\es'_\ell)][(\pi(\es_1), \pi(\es_2))$ and, therefore, $\T
  \models \rho[\es'_1, \ldots, \es'_\ell](\es_1, \pi^2(\es_1))$ since
  $\pi(\es'_j) = \es'_j$ for every $j \in \{1, \ldots, \ell\}$, $\es_2
  = \pi(\es_1)$ and $\rho(x, y)$ represents a strict partial order. In
  the same way, it is possible to conclude that $\T \models
  \rho[\es'_1, \ldots, \es'_\ell](\es_1, \pi^k(\es_1))$ for every $k
  \geq 1$. Given that the set of permutations of $n$ elements with the
  composition operator forms a group of order $n!$, we know that
  $\pi^{n!}$ is the identity permuntation, so that $\pi^{n!}(\es_1) =
  \es_1$. Therefore, we conclude that $\T \models \rho[\es'_1, \ldots,
    \es'_\ell](\es_1, \es_1)$, which leads to a contradiction since
  $\rho[v_1, \ldots, v_\ell](x,y)$ represents a strict partial order.
\end{proof}




